Quantum Meets the Minimum Circuit Size Problem

In this work, we initiate the study of the Minimum Circuit Size Problem (MCSP) in the quantum setting. MCSP is a problem to compute the circuit complexity of Boolean functions. It is a fascinating problem in complexity theory -- its hardness is mysterious, and a better understanding of its hardness can have surprising implications to many fields in computer science. We first define and investigate the basic complexity-theoretic properties of minimum quantum circuit size problems for three natural objects: Boolean functions, unitaries, and quantum states. We show that these problems are not trivially in NP but in QCMA (or have QCMA protocols). Next, we explore the relations between the three quantum MCSPs and their variants. We discover that some reductions that are not known for classical MCSP exist for quantum MCSPs for unitaries and states, e.g., search-to-decision reduction and self-reduction. Finally, we systematically generalize results known for classical MCSP to the quantum setting (including quantum cryptography, quantum learning theory, quantum circuit lower bounds, and quantum fine-grained complexity) and also find new connections to tomography and quantum gravity. Due to the fundamental differences between classical and quantum circuits, most of our results require extra care and reveal properties and phenomena unique to the quantum setting. Our findings could be of interest for future studies, and we post several open problems for further exploration along this direction.

==> main-qobjects.tex <==
\section{MCSP for Quantum Objects}\label{sec:main-qobjects}

%Finally, we discuss the $\MCSP$ analog for quantum objects. We first consider the $\MCSP$ for implementing a unitary transformation, which is the $\UMCSP$ problem. We study its complexity properties and the relation to $\MQCSP$. We also study the state preparation version of $\MCSP$, which is the $\SMCSP$ problem. 

%For technical reasons, we have to work on $\UMCSP$ and $\SMCSP$ with \textit{error gap parameters}. Namely, $\UMCSP_{\alpha,\beta}$ and $\SMCSP_{\alpha,\beta}$ where $\alpha$ and $\beta$ replace the $2/3$ and $1/2$ in Definition~\ref{def:umcsp_informal} and Definition~\ref{def:smcsp_informal}. The following theorems show upper bounds for $\UMCSP$ and $\SMCSP$ when the gap $|\alpha-\beta|$ is large enough.





\begin{theorem}
Let $\alpha,\beta\in(0,1)$ be the error gap parameters that potentially depend on $n$. When $1-\alpha< 2^{-2n-20}(1-\beta)^4$ and $1-\beta=\poly(1/2^n)$ (e.g., $1-\alpha=\mathsf{exp}(-2^n),1-\sqrt{\beta}=\poly(1/2^n)$), 
 $\UMCSP_{\alpha,\beta}\in\class{QCMA}$.
\end{theorem}



\begin{theorem}\label{thm:main_SQCMA_UMCSP}
$\SMCSP_{\alpha,\beta}$ has $\class{QCMA}$ proof with $|\alpha-\beta|\geq1/\poly(s)$. 
\end{theorem}

And we show the following reduction from $\MQCSP$ to $\UMCSP$:%\jyz{I changed the notation to the subscript}
%\nai{It is approximation ratio about circuit size, no the promise gap. I will make it clear in the context. }
\begin{theorem}\label{thm:main_b2u}
$\class{MQCSP}[\frac{s}{2}-1,s] \leq \class{UMCSP}$. 
\end{theorem}

%Combining this relation with previous theorems, we get the following corollaries.

By using this relation, several results about $\MQCSP$ in Section~\ref{sec:main-connections} also hold for $\UMCSP$. See Section~\ref{sec:quantum obj} for details. 
%\begin{corollary}
%If $\UMCSP\in \class{BQP}$, then there is no $\class{qOWF}$. 
%\end{corollary}


\subsection{Search-to-decision reductions}
Interestingly, we find that there are search-to-decision reductions for $\UMCSP$ and $\SMCSP$.



\begin{restatable}{theorem}{stdumcsp}\label{thm:search2decision_umcsp}
When the number of ancilla qubits $t$ is $O(n)$, there exists a search-to-decision reduction for $\class{UMCSP}$.
\end{restatable}
\vspace{-3mm}
\begin{restatable}{theorem}{stdsmcsp}\label{thm:s2d_smcsp}
There is a search-to-decision reduction for $\class{SMCSP}$. 
\end{restatable}

\begin{remark}
Since we define $\SMCSP$ and $\UMCSP$ as promise problems, the search-to-decision reductions only work when the instances satisfying the promises. On the other hand, if one consider $\SMCSP$ and $\UMCSP$ as decision problems (languages), then the search-to-decision reductions work for any instance. 
\end{remark}


It is unknown whether there is a search-to-decision reduction for the classical $\MCSP$ or not. Furthermore, we also don't know whether $\MQCSP$ has a search-to-decision reduction.  


\subsection{Applications of \texorpdfstring{$\SMCSP$}{SMCSP}}
We further study $\SMCSP$ and get the following results. We first relate $\SMCSP$ to the existence of pseudorandom states \cite{JLF18} and quantum-secure one-way functions:
\begin{theorem}
If $\SMCSP\in \class{BQP}$, then there are no pseudorandom states and $\class{qOWF}$. 
\end{theorem}
And we show how this problem is related to estimating the wormhole volume:
\begin{theorem}
Assuming the Volume=Complexity Conjecture and that the dictionary map can be computed in quantum polynomial time, when the wormhole's volume is polynomially large, $\SMCSP\in \class{BQP}$ if and only if there is a quantum polynomial time algorithm for estimating the wormhole's volume.
\end{theorem}
Finally, we show that solving the $\SMCSP$ can help to have a succinct answer to state tomography for states which are generated from a polynomial-size circuit without any measurement.   
\begin{definition}[Succinct state tomography]
\label{def:main_sst}
Let $\ket{\psi}$ be an $n$-qubit quantum state that is generated from a quantum circuit $\Circ$ of size $s$ without any measurement. Given $\poly(n)$ copies of $\ket{\psi}$ and an upper bound $s' $ where $s\leq s'\leq \poly(n)$, the goal is to output a succinct description (e.g., $\Circ$) of $\ket{\psi}$.  
\end{definition}
\begin{theorem}\label{thm:sst}
Succinct state tomography in Definition~\ref{def:main_sst} reduces to the $\SMCSP$.   
\end{theorem}

%The formal statements and proofs are deferred to Section~\ref{sec:smcsp_app}.

==> table-2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|}
\hline
                          & Results                                                                                                                    & \makecell{Informal Theorem Index\\ (Formal Theorem Index)}                          \\ \hline
\multirow{12}{*}{\makecell{$\MQCSP$\\(Def.~\ref{def:main_bmcsp})}} & $\MQCSP\in\class{QCMA}$                                                                                                     & Theorem~\ref{thm:informal_mqcsp_crypto}  (Theorem~\ref{thm:QCMA_MCSP})                           \\ \cline{2-3}
& $\MQCSP\in\class{BQP}$ $\Rightarrow$ No \textsf{qOWF}                                                                       & Theorem~\ref{thm:informal_mqcsp_crypto}  (Theorem~\ref{thm:mqcsp_qowf})                           \\ \cline{2-3}
& $\class{SZK}\leq \MQCSP$                                                            & Theorem~\ref{thm:informal_mqcsp_crypto}  (Theorem~\ref{thm:szk_mcsp})                           \\ \cline{2-3}
& $\mBMCSP$ is $\class{NP}$-hard    under a natural gate set                                                                 & Theorem~\ref{thm:informal_mqcsp_crypto}  (Theorem~\ref{thm:mqcsp_multi hard})                           \\ \cline{2-3}
& $i{\cal O}+\MQCSP\in\class{BQP}$ $\Rightarrow$ $\class{NP}\subseteq\class{coRQP}$   & Theorem~\ref{thm:informal_mqcsp_crypto}  (Theorem~\ref{thm:qioimplication})                           \\ \cline{2-3}
& PAC learning for $\class{BQP/poly}$ $\Leftrightarrow$ $\MQCSP\in\class{BPP}$                                                & Theorem~\ref{thm:pac_informal}  (Theorem~\ref{thm:PAC learning and MQCSP})                           \\ \cline{2-3}
& $\class{BQP}$ learning $\Leftrightarrow$ $\MQCSP\in \class{BQP}$                                                           & Theorem~\ref{thm:learning_informal}  (Theorem~\ref{thm:quantum learning MCSP})                           \\ \cline{2-3}
& $\MQCSP\in\class{BQP}\Rightarrow \class{BQE}\not\subset\class{BQC}[n^k],\ \forall k\in\mathbb{N}_+$ & Theorem~\ref{thm:informal_circuit_lb}  (Theorem~\ref{thm:ckt lb from MQCSP in BQP max})                           \\ \cline{2-3}
& $\MQCSP\in\class{BQP}\Rightarrow \class{BQP^{QCMA}}\not\subset\class{BQC}[n^k],\ \forall k\in\mathbb{N}_+$ & Theorem~\ref{thm:informal_circuit_lb}  (Theorem~\ref{thm:magnification})                           \\ \cline{2-3}
& $\MQCSP\in\class{BQP}$ $\Rightarrow$ Hardness amplification                                                                 & Theorem~\ref{thm:amp_intro}  (Theorem~\ref{thm:mqcsp_hardness_amp})                           \\ \cline{2-3}
& Hardness magnification for $\class{MQCSP}$                                                                & Theorem~\ref{thm:magnify_informal}  (Theorem~\ref{thm:magnification})                           \\ \cline{2-3}
& $\class{QETH}\Rightarrow$ quantum hardness of $\MQCSP^\star$                                   & Theorem~\ref{thm:mqcsps_informal}  (Theorem~\ref{thm:qeth_hard_mqcsps})                           \\ \hline                          
                          
\multirow{7}{*}{\makecell{$\UMCSP$\\(Def.~\ref{def:umcsp})}} & $\UMCSP\in\class{QCMA}$                                                                                                    & Theorem~\ref{thm:smcspumcspqcma}  (Theorem~\ref{thm:umcspqcma})                                  \\ \cline{2-3} 
                          & Search-to-decision reduction for $\UMCSP$                                                                      & Theorem~\ref{thm:informal_reduction}  (Theorem~\ref{thm:search2decision_umcsp})                              \\ \cline{2-3} 
                          & $\textsf{gap}$-$\MQCSP\leq\UMCSP$                                                                                          & Theorem~\ref{thm:informal_reduction}  (Theorem~\ref{thm:b2u})                              \\ \cline{2-3} 
                          & \makecell{$\UMCSP\in\class{BQP}$ \\ $\Rightarrow$ No pseudorandom unitaries and no \textsf{qOWF}}                          &  (Theorem~\ref{thm:pru}, Corollary~\ref{cor:umcsp_owf}) \\ \cline{2-3} 
                          &$i\mathcal{O}+\UMCSP\in\class{BQP}$ $\Rightarrow$ $\class{NP}\subseteq\class{coRQP}$ & (Corollary~\ref{cor:umcsp_io})                                                      \\ \cline{2-3} 
                          & $\UMCSP\in\class{BQP}$ $\Rightarrow$ Hardness amplification for $\class{BQP}$                                              & (Corollary~\ref{cor:umcsp_amp})                                                     \\ \cline{2-3} 
                          & $\UMCSP\in\class{BQP}$ $\Rightarrow$ $\class{BQE}\not\subset\class{BQP}[n^k],\ \forall k\in\mathbb{N}$                     & (Corollary~\ref{cor:umcsp_bqe})                                                     \\ \hline
\multirow{6}{*}{\makecell{$\SMCSP$\\(Def.~\ref{def:smcsp})}} & $\SMCSP$ can be verified via $\class{QCMA}$                                                                                & Theorem~\ref{thm:smcspumcspqcma}  (Theorem~\ref{thm:SQCMA_UMCSP})                                  \\ \cline{2-3} 
                          & Search-to-decision reduction for $\SMCSP$                                                                      & Theorem~\ref{thm:informal_reduction}  (Theorem~\ref{thm:s2d_smcsp})                              \\ \cline{2-3} 
                          & Self-reduction for $\SMCSP$                                                                                    & Theorem~\ref{thm:informal_reduction}  (Theorem~\ref{thm:smcsp_self_reduction})                              \\ \cline{2-3} 
                          & \makecell{$\SMCSP\in\class{BQP}$ \\ $\Rightarrow$ No pseudorandom states and no \textsf{qOWF}}                             & Theorem~\ref{thm:smcsp_app_informal}  (Theorem~\ref{thm:smcsp_no qOWF})                              \\ \cline{2-3} 
                          & \makecell{Assume conjectures from physics\\ $\SMCSP$ $\Leftrightarrow$ Estimating wormhole's volume}                       & Theorem~\ref{thm:smcsp_app_informal}  (Theorem~\ref{thm:smcsp_wormwhole})                              \\ \cline{2-3} 
                          & Succinct state tomography $\leq \SMCSP$                            & Theorem~\ref{thm:smcsp_app_informal}  (Theorem~\ref{thm:smcsp_succinct tomo})                              \\ \hline
\end{tabular}
\caption{Summary of our results.}
\label{tab:UMCSP SMCSP}
\end{table}

==> table.tex <==
\begin{table}[]
\centering
\begin{tabular}{|c|c|}
\hline
Result                                                                                                                      & \makecell{Informal Theorem Index\\ (Formal Theorem Index)} \\ \hline
$\MQCSP\in\class{QCMA}$                                                                                                     & Theorem~\ref{thm:informal_mqcsp_crypto}  (Theorem~\ref{})                           \\ \hline
$\MQCSP\in\class{BQP}$ $\Rightarrow$ No \textsf{qOWF}                                                                       & Theorem~\ref{thm:informal_mqcsp_crypto}  (Theorem~\ref{})                           \\ \hline
$\class{SZK}\leq \MQCSP$                                                            & Theorem~\ref{thm:informal_mqcsp_crypto}  (Theorem~\ref{})                           \\ \hline
$i{\cal O}+\MQCSP\in\class{BQP}$ $\Rightarrow$ $\class{NP}\subseteq\class{coRQP}$   & Theorem~\ref{thm:informal_mqcsp_crypto}  (Theorem~\ref{})                           \\ \hline
$\mBMCSP$ is $\class{NP}$-hard under a natural gate set                                                                     & Theorem~\ref{thm:informal_mqcsp_crypto}  (Theorem~\ref{})                           \\ \hline
PAC learning for $\class{BQP/poly}$ $\Leftrightarrow$ $\MQCSP\in\class{BPP}$                                                & Theorem~\ref{thm:pac_informal}  (Theorem~\ref{})                           \\ \hline
$\class{BQP}$ learning $\Leftrightarrow$ $\MQCSP\in \class{BQP}$                                                           & Theorem~\ref{thm:learning_informal}  (Theorem~\ref{})                           \\ \hline
$\MQCSP\in\class{BQP}\Rightarrow \class{BQE}\not\subset\class{BQP/poly}$ & Theorem~\ref{thm:informal_circuit_lb}  (Theorem~\ref{})                           \\ \hline
$\MQCSP\in\class{BQP}\Rightarrow \class{BQP^{QCMA}}\not\subset\class{BQP/poly}$ & Theorem~\ref{thm:informal_circuit_lb}  (Theorem~\ref{})                           \\ \hline
$\MQCSP\in\class{BQP}$ $\Rightarrow$ Hardness amplification                                                                 & Theorem~\ref{thm:amp_intro}  (Theorem~\ref{})                           \\ \hline
Hardness magnification for $\class{MQCSP}$                                                                & Theorem~\ref{thm:magnify_informal}  (Theorem~\ref{})                           \\ \hline
$\class{QETH}\Rightarrow$ quantum hardness of $\MQCSP^\star$                                   & Theorem~\ref{thm:mqcsps_informal}  (Theorem~\ref{})                           \\ \hline
\end{tabular}
\caption{Summary of our results on $\MQCSP$.\cnc{Fill up indices later.}}
\label{tab:MQCSP}
\end{table}
